Approximating the Shapley Value of Minimum Cost Spanning Tree Games: An FPRAS for Saving Games

In this research, we address the problem of computing the Shapley value in minimum-cost spanning tree (MCST) games. We introduce the saving game as a key framework for approximating the Shapley value. By reformulating MCST games into their saving-game counterparts, we obtain structural properties that enable multiplicative (relative-error) approximation. Building on this reformulation, we develop a Monte Carlo based Fully Polynomial-time Randomized Approximation Scheme (FPRAS) for the Shapley value.

==> Proofs-old/FPRAS.tex <==
\begin{proof}
% Obviously, 
%we have $\Exp [\phi^A_i]=\phi_i$ $(\forall i \in N)$.
For each $m \in \{1, 2, \ldots, M\}$ and $i \in N$, 
    define the random variable 
    $\Delta^{(m)}_i = \Merg(\pi, i)$, 
    where $\pi \in \Pi_N$ is 
    the permutation sampled 
    in the $m$-th iteration of Algorithm~\ref{algo1}.
As Algorithm~\ref{algo1} chooses a permutation $\pi \in \Pi_N$ randomly, 
    it is obvious that for each player $i \in N$, 
	$\{ \Delta^{(1)}_i, \Delta^{(2)}_i, \ldots , \Delta^{(M)}_i\}$ 
	is a Bernoulli process satisfying
	$\phi^A_i=\sum_{m=1}^M \Delta^{(m)}_i/M$ and 
 	$ \Exp \left[ \phi^A_i \right]
	=\Exp \left[ \Delta^{(m)}_i \right]=\phi_i$ 
	$(\forall m \in \{1,2,\ldots ,M\})$.

%We define $\widetilde{w_i}=\min \{w_i , W-w_0\}$.
%Obviously, the inequalities $ 0\leq \Merg (\pi, i) \leq \widetilde{w_i}$ hold for any $(\pi, i) \in \Pi_N \times N$.
%Thus, the range of random variable $\Delta^{(m)}_i$ is contained in the interval $[0, \widetilde{w_i}]$. 
% Additionally, the Shapley value satisfies that 
% \[
%  \phi_i
%  = \frac{1}{n!} \sum_{\pi \in \Pi_N} \Merg (\pi ,i)
%  \geq \frac{1}{n!} \sum_{\pi \in \Pi_N: \pi (n)=i} \Merg (\pi ,i)
%  =\frac{(n-1)!}{n!} \widetilde{w_i} 
%  =\frac{\widetilde{w_i}}{n} \;\;\;
%  (\forall i \in N).
% \]
The definition of Algorithm~\ref{algo1}
    directly implies that 
    $\Delta^{(m)}_i \in [0, w_i]$ $(\forall i \in N).$
In addition, 
    Assumption~\ref{Assumption:wi<E}  ensures that  
    $\Merg (\pi, i) = w_i$ holds
    for any $(\pi, i) \in \Pi_N \times N$
    such that $\pi (n)=i.$
Thus, we obtain a lower bound for 
    the Shapley value, satisfying 
\[
 \phi_i
 = \frac{1}{n!} \sum_{\pi \in \Pi_N} \Merg (\pi ,i)
 \geq \frac{1}{n!} \sum_{\pi \in \Pi_N: \pi (n)=i} 
    \Merg (\pi ,i)
 =\frac{(n-1)!}{n!} w_i 
 =\frac{w_i}{n} (>0)  \;\;\;
 (\forall i \in N).
\]



Hoeffding's inequality~\cite{hoeffding1963probability}
	implies that 
	each player $i \in N$ satisfies
\begin{eqnarray*}
\Prob \left[ \left| \phi^A_i
	- \Exp \left[ \phi^A_i \right] \right|
	\geq t \right]
&\leq 
& 2 \exp \left(
	- \frac{2M^2 t^2}{\sum_{m=1}^M ({w_i}-0)^2}
	\right)
= 2 \exp \left( \frac{-2M t^2}{{w_i}^2} \right).
\end{eqnarray*}

(1) If we set 
	$\displaystyle M \geq \frac{n^2 \ln (2/\delta)}{2\varepsilon^2}$,
	then 
\[
\begin{array}{l}
\displaystyle 
\Prob 
	\left[ 
		\frac{| \phi^A_i-\phi_i| }{\phi_i}
            < \varepsilon  
	\right] 
=
\Prob 
	\left[ 
		\left| \phi^A_i-\Exp \left[ \phi^A_i \right] \right| 
            < \varepsilon  \phi_i
	\right] 
\geq \Prob 
	\left[ 
		\left| \phi^A_i-\Exp \left[ \phi^A_i \right] \right| 
            < \varepsilon  \left( \frac{{w_i}}{n} \right) 
	\right]  \\
\displaystyle 
= 1- \Prob 
	\left[ 
		\left| \phi^A_i-\Exp \left[ \phi^A_i \right] \right| 
            \geq \left( \frac{\varepsilon {w_i}}{n} \right)
	\right]  
\geq 1- 
2 \exp \left( \frac{-2M (\varepsilon {w_i}/n)^2}{{w_i}^2} \right)\\
\displaystyle 
=1- 
2 \exp \left( -M \frac{2  \varepsilon^2}{n^2} \right)
\geq  
1- 2 \exp \left( - \ln \left( \frac{2}{\delta} \right) \right) =
  1-\delta.
 \end{array}
\] 

(2) If we set 
	$\displaystyle M\geq \frac{n^2 \ln (2n/\delta)}{2\varepsilon^2}$,
	then we have that
\[
\begin{array}{l}
\displaystyle 
\Prob \left[
				\forall i \in N, 
					\frac{\left| 
						\phi^A_i	- \varphi_i 
					\right|}{\phi_i}
					< \varepsilon 
			\right]
 = 1- \Prob 
			\left[
				\exists i \in N, 
					\left|
                        \phi^A_i-\Exp \left[ \phi^A_i \right] 
                    \right| 
					\geq \varepsilon \phi_i
			\right] \\
\displaystyle
 \geq 
 1-\sum_{i \in N} 
	\Prob 
			\left[
					\left|
                        \phi^A_i-\Exp \left[ \phi^A_i \right] 
                    \right| 
					\geq \varepsilon \phi_i
			\right]
\geq 
1-\sum_{i \in N} 
	\Prob 
			\left[
					\left|
                        \phi^A_i-\Exp \left[ \phi^A_i \right] 
                    \right| 
					\geq \varepsilon \left( \frac{{w_i}}{n} \right)
			\right] \\
\displaystyle 
\geq 1- \sum_{i=1}^n  2 \exp 
        \left( 
            \frac{-2M (\varepsilon {w_i} /n)^2 }{{w_i}^2}
        \right) 
\geq 1- \sum_{i=1}^n  2 \exp 
        \left( -M 
            \frac{2 \varepsilon^2 }{n^2}
        \right) \\
\displaystyle
 \geq 
 1- \sum_{i=1}^n  2 \exp 
	\left( 
		- \ln \left( \frac{2n}{\delta} \right) 
 	\right) 
= 1-\sum_{i=1}^n \frac{\delta}{n}=1-\delta.  
\end{array}
\]
\end{proof}

==> Proofs-old/NPC.tex <==
\begin{proof}
(1) Problem SHP belongs to the class NP.

We show that $\phi_n < \frac{1}{2}$ if and only if 
  $\exists \pi \in \Pi_N$ satisfying $\Merg (\pi, n) + \Merg (\pi^{\textup{R}}, n) <1$.
Lemma~\ref{Theorem:w_0Monotone} and Corollary~\ref{Theorem:CorMerg}  imply that 
\[
  \Merg (\pi, n)+\Merg (\pi^{\textup{R}}, n) 
  \leq \MergH (\pi, n) + \MergH(\pi^{\textup{R}}, n) = w_n=1.
\] 
Thus, we have that 
\[
\phi_n = \frac{1}{n!} \sum_{\pi \in \Pi_N} \Merg (\pi ,n)
    =\frac{1}{2\cdot n!} \sum_{\pi \in \Pi_N} 
        (\Merg (\pi ,n)+ \Merg(\pi^{\textup{R}}, n))
        \leq  \frac{1}{2\cdot n!} \sum_{\pi \in \Pi_N} 1  =\frac{1}{2}.
\]
The above properties directly imply that 
    $\phi_n =(1/2)$
    if and only if 
    \mbox{$\Merg (\pi ,n)+ \Merg (\pi^{\textup{R}}, n)=1$}
    holds for any $\pi \in \Pi_N$.
Now we have a desired result and 
    a permutation $\pi$ satisfying 
     \mbox{$\Merg (\pi ,n)+ \Merg (\pi^{\textup{R}}, n)< 1$}  
     is a polynomial size certificate when problem SHP has YES answer.
 

\smallskip 
\noindent
(2) We show that the known NP-complete problem PARTITION can be reduced to problem SHP in polynomial time.



\[
\fbox{\parbox{0.9\textwidth}{
\textbf{PARTITION Problem}\\
\textbf{Instance:} 
%A positive integer $n\in \mathbb{Z}_+$ and a 
A positive integer vector 
 $(a_1, \dots, a_m)$. \\
\textbf{Question:} 
Does there exist a subset $S \subseteq \{1,2,\ldots ,m\}$ satisfying 
$\displaystyle 
 \sum_{i \in S}a_i %= \sum_{i \in A\backslash S}a_i 
   = \frac{1}{2}\sum_{i=1}^m a_i$?
}}
\]
We construct an instance of problem SHP from that of PARTITION as follows:
we set  $n = m+1$, % and 
\[
w_i = \left\{ \begin{array}{ll}
   2a_i & (i \in \{1,2,\dots, n-1\}), \\
   1     & (i=n=m+1),
   \end{array} \right. \mbox{ and }  
w_0 =  \frac{1}{2} \sum_{i=1}^{n-1} w_i + 1  
= \sum\limits_{i=1}^{m} a_i + 1.
\]
Now, we prove that the PARTITION problem instance has YES answer if and only if the answer to problem SHP instance is Yes.

\noindent\underline{
[PARTITION has Yes answer $\Rightarrow$ SHP has Yes answer]
}

As problem PARTITION has  Yes answer, 
 there exists $S \subseteq \{1,2,\ldots ,n-1\}$ 
 satisfying $\sum_{i \in S} a_i =  \frac{1}{2}\sum_{i=1}^{m}a_i$. 
We construct a permutation $\pi_{*} \in \Pi_N$ 
 satisfying $\Prec (\pi_{*}, n)=S$.
Then, it is easy to see that 
\[
% w(\Prec(\pi_{*}, n)) <
 w(\Prec(\pi_{*}, n)\cup \{n\}) 
 =\frac{1}{2}\sum_{i=1}^{m}a_i +1
 = w_0.
 \]
Thus, we have that 
\[
\Merg (\pi_{*}, n) %+ \Merg (\pi_{*}^{\textup{R}}, n)
=v(\Prec(\pi_{*}, n)\cup \{n\})- v(\Prec(\pi_{*}, n))  ) =0-0=0.
\]
Similarly, the equalities 
\[
% w(\Prec(\pi_{*}^{\textup{R}}, n)) <
 w(\Prec(\pi_{*}^{\textup{R}}, n)\cup \{n\}) 
 =\frac{1}{2}\sum_{i=1}^{m}a_i +1
 = w_0
\]
imply that 
\[
\Merg (\pi_{*}^{\textup{R}}, n) %+ \Merg (\pi_{*}^{\textup{R}}, n)
=(v(\Prec(\pi_{*}^{\textup{R}}, n)\cup \{n\})- v(\Prec(\pi_{*}^{\textup{R}}, n))  ) 
 =0-0=0.
\]
As shown in (1), the inequality 
\[
\Merg (\pi_{*}, n)+ \Merg (\pi_{*}^{\textup{R}}, n)
    =0+0 =0 <1
\]
implies $\phi_n < \frac{1}{2}$. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent\underline{
[SHP has Yes answer $\Rightarrow$ PARTITION has Yes answer]
}

In the following, we show the contraposition.
Assume that PARTITION has NO answer, i.e., 
    $\forall S \subseteq \{1,2,\ldots n-1\},$
    $w(S) \neq (1/2)\sum_{i=1}^{n-1} w_i$.
We only need to show that $\forall \pi \in \Pi_N$, 
    $\Merg (\pi, n)+\Merg (\pi^{\textup{R}},n)=1$.
    
For any permutation $\pi \in \Pi_N$, we have the following.
The assumption implies that  $w(\Prec (\pi, n)) \neq (1/2)\sum_{i=1}^{n-1} w_i$.
Consider the case that $w(\Prec (\pi, n)) < (1/2)\sum_{i=1}^{n-1} w_i$.
As $\{w_1, w_2, \ldots ,w_{n-1}\}$ is a set of even integers, 
the inequality  $w(\Prec (\pi, n)) \leq  (1/2)\sum_{i=1}^{n-1} w_i -1$ holds.
Thus, we have that
\[
    w(\Prec (\pi, n)) \leq  w(\Prec (\pi, n)\cup \{n\}) 
    = w(\Prec (\pi, n)) +1 \leq  (1/2)\sum_{i=1}^{n-1} w_i =w_0,
\]
which leads to the equality
\[
    \Merg (\pi, n)=v (\Prec (\pi,n) \cup \{n\})-v(\Prec (\pi, n))=0-0=0.
\]
Similarly, we have that 
\[
\begin{array}{r@{}l}
  w(\Prec (\pi^{\textup{R}}, n) \cup \{n\}) 
  & \geq w(\Prec (\pi^{\textup{R}}, n))   
  = (W-w(\Prec(\pi ,n) \cup \{n\})) \\
  &\displaystyle 
    =\sum_{i=1}^{n-1}w_i+1 -( w(\Prec(\pi ,n)) +w_n) \\
  &\displaystyle 
    \geq  \sum_{i=1}^{n-1}w_i+1- ((1/2) \sum_{i=1}^{n-1}w_i -1) -w_n
 = (1/2) \sum_{i=1}^{n-1}w_i +1 = w_0,
\end{array}
\]
which leads to the equality
\[
\begin{array}{r@{}l}
 \Merg (\pi^{\textup{R}}, n)
 &=v (\Prec (\pi^{\textup{R}},n) \cup \{n\})-v(\Prec (\pi^{\textup{R}}, n)) \\
 &=(-w_0+ w(\Prec (\pi^{\textup{R}},n)\cup \{n\})) 
 -(-w_0+ w(\Prec (\pi^{\textup{R}},n))) \\
 &= w(\Prec (\pi^{\textup{R}},n))+w_n - w(\Prec (\pi^{\textup{R}},n))=1.
\end{array} 
\]
From the above, the equality   $\Merg (\pi, n)+\Merg (\pi^{\textup{R}},n)=1$ holds.
In a similar way, we can deal with the remaining case that 
    $w(\Prec (\pi, n)) > (1/2)\sum_{i=1}^{n-1} w_i$.
\end{proof}



==> Proofs-old/PropDist.tex <==

\begin{proof}
In this proof, we discuss the game  $(N,\vHalf)$
    defined by $\ReL [\frac{W}{2}; \Vec{w}]$, 
    which is equal to $\BG[\frac{W}{2}; \Vec{w}].$
We define %$w_0=\frac{1}{2}W$  %,  
% $\Hprop{\Vec{y}}=(w_1/2, w_2/2, \ldots ,w_n/2)$ and 
 $\MergH (\pi, i)
     = \vHalf (\Prec (\pi, i) \cup \{i\}) -\vHalf (\Prec(\pi, i))$
%for each pair 
$(\forall (\pi, i) \in \Pi_N \times N)$
and
$w_0=\frac{1}{2}W.$
For any permutation $\pi \in \Pi_N$, 
 we denote its reverse permutation by $\pi^\textup{R}$.

In the following, we show that
\[
  \MergH (\pi, i)+\MergH (\pi^\textup{R}, i)=w_i \quad (\forall i \in N).
\]
%\vskip 5pt
by considering  the following three cases;

\vskip 5pt

\begin{enumerate}[label=Case~\arabic*:, leftmargin=*]
  \item $w (\Prec (\pi, i) \cup \{i\}) < w_0,$
  \item $w(\Prec (\pi^\textup{R} ,i)\cup \{i\}  ) < w_0,$
  \item $w (\Prec (\pi, i) \cup \{i\}) \geq w_0$ and
        $w(\Prec (\pi^\textup{R} ,i)\cup \{i\}  ) \geq w_0.$
\end{enumerate}

\vskip 5pt
\noindent
\underline{Case~1}: Let consider the case that $w (\Prec (\pi, i) \cup \{i\}) < w_0$. 
Then, the marginal contribution satisfies 
\[
    \MergH (\pi, i) 
    = \vHalf (\Prec (\pi ,i)\cup \{i\}) - \vHalf (\Prec (\pi ,i))
    =0-0=0.
\]
The reverse permutation $\pi^\textup{R}$ satisfies that
\[
\begin{array}{r@{ }l}
 -w_0 + w(\Prec (\pi^\textup{R},i))
 &= -w_0 + w(N \setminus (\Prec (\pi ,i) \cup \{i\}))
 = -w_0 + w(N)-w(\Prec (\pi ,i) \cup \{i\}) \\
 &> -w_0 +W -w_0 = W -2w_0=W-W=0
 \end{array}
\]
and thus, 
\[
\begin{array}{r@{ }l}
 \MergH (\pi^\textup{R}, i) 
    &= \vHalf (\Prec (\pi^\textup{R} ,i)\cup \{i\}) 
    - \vHalf (\Prec (\pi^\textup{R} ,i)) \\
    &=-w_0 + w (\Prec(\pi^\textup{R} ,i)\cup \{i\} )
    -(-w_0 + w(\Prec(\pi^\textup{R} ,i))) \\
    &=w(\Prec(\pi^\textup{R} ,i))+w_i - w(\Prec(\pi^\textup{R} ,i))=w_i.
\end{array}
\]
We obtain that  $\MergH (\pi, i)+\MergH (\pi^\textup{R}, i)=w_i$.

\vskip 5pt
\noindent
\underline{Case~2}: When $w(\Prec (\pi^\textup{R} ,i)\cup \{i\}  ) < w_0$, 
 we can prove the desired equality similarly to Case 1 by swapping $\pi$ and 
 $\pi^\textup{R}$.

\vskip 5pt
\noindent
\underline{Case 3}: 
Consider the remained case that both
$w (\Prec (\pi, i) \cup \{i\}) \geq w_0$ and
 $w(\Prec (\pi^\textup{R} ,i)\cup \{i\}  ) \geq w_0$ hold. 
The assumption directly implies 
\[
\begin{array}{r@{ }l}
\vHalf (\Prec (\pi, i) \cup \{i\})
=-w_0 +w(\Prec (\pi, i) \cup \{i\}) 
= -w_0 +w(\Prec (\pi, i))+w_i 
\end{array}
\]
and
\[
\begin{array}{r@{ }l}
\vHalf (\Prec (\pi^\textup{R}, i) \cup \{i\})
&=-w_0 +w(\Prec (\pi^\textup{R}, i) \cup \{i\}) 
= -w_0 +w(N \setminus \Prec (\pi, i)) \\
&= -w_0 +W - w(\Prec (\pi, i)).
\end{array}
\]
We also obtain that 
\[
\begin{array}{r@{ }l}
w(\Prec (\pi, i) )
=w(N\setminus ( \Prec(\pi^\textup{R}, i) \cup \{i\})
=W - w( \Prec(\pi^\textup{R}, i) \cup \{i\})\leq W-w_0=W-W/2=w_0
\end{array}
\]
and thus 
\[
\vHalf (\Prec (\pi, i) )= \max \{0, -w_0+w(\Prec (\pi, i))=0.
\]
Similarly, we have that 
$\vHalf (\Prec (\pi^\textup{R}, i) )=0.$

The above properties result in the following 
\[
\begin{array}{r@{ }l}
\MergH (\pi, i)+\MergH (\pi^\textup{R}, i)
&= \vHalf (\Prec (\pi, i) \cup \{i\}) - w(\Prec (\pi, i) )
+\vHalf (\Prec (\pi^\textup{R}, i) \cup \{i\}) - \vHalf (\Prec (\pi^\textup{R}, i) ) \\
&=(-w_0 +w(\Prec (\pi, i))+w_i) -0
 +(-w_0 +W - w(\Prec (\pi, i)))-0 \\
 &=-2w_0+W +w_i =w_i.
\end{array}
\]

The Shapley value $\phi_i$ of player $i$ satisfies
\begin{align*}
\phi_i &= \frac{1}{n!}\sum_{\pi \in \Pi_N} \MergH (\pi, i) 
=\frac{1}{2\cdot n!}\sum_{\pi \in \Pi_N}(\MergH (\pi, i) + \MergH (\pi^{\textup{R}}, i) )
=\frac{1}{2\cdot n!}\sum_{\pi \in \Pi_N}w_i 
% = \frac{n!}{2 \cdot n!}w_i 
 =\frac{1}{2}w_i.
\end{align*}
\end{proof}



==> Proofs-old/PropVecCore.tex <==
\begin{proof}
As $\Hprop{\Vec{y}}$ is an imputation, we only need to show that it satisfies coalitional rationality 
 $[\sum_{i \in S}y_i \geq v(S) \; (\forall S \subseteq N)]$.

\begin{enumerate}
    \item If $\sum_{i \in S} w_i < w_0$,
 then the non-negativity of $\Hprop{\Vec{y}}$ implies $\sum_{i \in S} \Hprop{y_i} \geq 0=v(S)$.
    \item In the remained case that $\sum_{i \in S} w_i \geq w_0$,
    we have the following inequalities
\[
    \sum_{i \in S} \Hprop{y_i} - v(S) 
    = \frac{W-w_0}{W}\sum_{i \in S} w_i 
       - \left( -w_0+\sum\limits_{i \in S}w_i \right) 
    =w_0 \left( 1-\frac{\sum_{i \in S}w_i}{W} \right) \geq 0.
\]
\end{enumerate}
%Therefore
%$\sum\limits_{i \in S}y_i \geq v(S) \;\;
%  (\forall S \subseteq N)$
%holds.
\end{proof}

==> Proofs-old/PropVecImp.tex <==
\begin{proof}
1. Each player $i \in N$ satisfies that $\Hprop{y_i} \geq 0$ and 
$ \Hprop{y_i} - (-w_0 + w_i) 
    = w_0 \left(1 - \frac{w_i}{W}\right) 
    \geq 0$. 
The above inequalities directly imply that 
 $ \Hprop{y_i} \geq \max \{0, -w_0+w_i \}=v(\{i\}).$

2. The definition of $\Hprop{\Vec{y}}$ directly implies that 
\[
\sum_{i \in N} \Hprop{y_i}
 = \frac{(W - w_0)}{W} \sum_{i \in N}w_i = W - w_0 = v(N).
\]
\end{proof}

==> Proofs-old/bankruptcy.tex <==
\begin{proof}
Let $(N, v)$ be a rectified linear function game with:
\begin{center}
$v(S) = \max \left\{ 0, -w_0 + \sum\limits_{i \in S} w_i \right\} $
\end{center}

Define a bankruptcy game $(N, E, d)$ where:
\begin{itemize}
\item $E = W - w_0 = \sum_{i \in N} w_i - w_0$
\item $d_i = w_i$ for all $i \in N$
\end{itemize}

For any coalition $S \subseteq N$, the value in the bankruptcy game is:
\begin{align*}
v_E^d(S) &= \max \left\{ 0, E - \sum\limits_{i \in N \setminus S} d_i \right\} 
 = \max \left\{ 0, (W - w_0) - \sum\limits_{i \in N \setminus S} w_i \right\} \\
&= \max \left\{ 0, W - w_0 - \left( W - \sum\limits_{i \in S} w_i \right) \right\} 
 = \max \left\{ 0, -w_0 + \sum\limits_{i \in S} w_i \right\} 
 = v(S)
\end{align*}

Conversely, given a bankruptcy game $(N, v_E^d)$, we can define a rectified linear function game with $w_i = d_i$ for all $i \in N$ and $w_0 = \sum\limits_{i \in N} d_i - E$. 
\end{proof}

==> Proofs-old/merg.tex <==
\begin{Lemma}\label{lemma:merg}
Consider a bankruptcy game defined by $[E; w_1, \ldots, w_n]$, 
and let $\Merg(\pi,i)$ denote the marginal contribution of player $i \in N$ 
for a permutation $\pi$ in this game.  

Similarly, consider a weighted voting game defined by $[q; w_1, \ldots, w_n]$, 
and let $\Mergq(\pi,i)$ denote the marginal contribution of player $i \in N$ 
for a permutation $\pi$ in this game.

Then, the following holds:
\[
\Merg(\pi,i) = \sum_{q = w_0+1}^{W}\Mergq(\pi,i),
\]
where $W = w_1 + \cdots + w_n$.
\end{Lemma}



\begin{proof}
It is obvious that $\Merg(\pi,i) = \sum_{q = w_0+1}^{W}\Mergq(\pi,i)=0$ holds when $w_i=0$.  
We now turn to the case $w_i > 0$. 

Let $s = \sum_{j \in \text{Prc}(\pi,i)} w_j$.  
We divide the proof into three cases depending on the value of $w_0$.



\item Case 1: $0 \le w_0 \le s$. \\
First, by the definition of $\Mergq$, we have
\[
\sum_{q=w_0+1}^W\Mergq(\pi,i)=\sum_{q=s+1}^{s+w_i}1 = w_i.
\]
In addition, we obtain
\begin{align*}
\Merg(\pi,i)& =\max(0,-w_0+s+w_i) - \max(0,-w_0+s) 
\\ &= (-w_0+w_i+s) - (-w_0+s) 
\\ &= w_i.
\end{align*}

\item Case 2: $s < w_0 < s+w_i$. \\
By the definition of $\Mergq$, we have
\[
\sum_{q=w_0+1}^W\Mergq(\pi,i)=\sum_{q=w_0+1}^{s+w_i}1 = -w_0+w_i+s.
\]
Also, 
\begin{align*}
\Merg(\pi,i)&=\max(0,-w_0+s+w_i) - \max(0,-w_0+s) 
\\&= (-w_0+w_i+s) - 0 
\\&= -w_0+w_i+s.
\end{align*}

\item Case 3: $s+w_i \le w_0 \le W$. \\
In this case, player $i$ cannot be a pivot player for any quota $q \in [w_0+1,W]$.  
Therefore,
\[
\sum_{q=w_0+1}^W\Mergq(\pi,i)=0.
\]
Moreover,
\[
\Merg(\pi,i)=\max(0,-w_0+s+w_i) - \max(0,-w_0+s) 
= 0 - 0 
= 0.
\]

This completes the proof.
\end{proof}


==> Proofs-old/recursiveL.tex <==
\begin{proof}
%    Omitted. (See~\cite{o1982problem,driessen1988cooperative}
%    for example.)

    It is obvious that 
    for every subset 
    $S'' \subseteq N$ such that  
    $|S''|\geq 2$ and  $\sum_{k\in S''}w_k>w_0$, 
    we have 
\[
    v^{[S'']} (S)
        =\max \left\{ 0, -w_0 +\sum_{k\in S} w_k \right\}
        =v(S) \;\; (\forall S \subseteq S'').
\]

If $|S'|\geq 2$ and  $\sum_{k\in S'}w_k > w_0,$
    then the Shapley value $\phi^{[S']}$ 
    satisfies that 
\begin{eqnarray*}
 \phi^{[S']}_i
 &=&
 \frac{1}{|S'|!}\sum_{\pi \in \Pi_{S'}} 
    \delta_{v^{[S']}}(\pi,i) 
  = \frac{1}{|S'|!} 
  \left( 
    \sum_{\pi \in \PrmL{S'}{i}} \delta_{v^{[S']}}(\pi,i) 
    + \sum_{j\in S' \setminus \{i\}} 
      \sum_{\pi \in \PrmL{S'}{j}} \delta_{v^{[S']}}(\pi,i) 
  \right) \\
  &=&\frac{1}{|S'|}
  \left( \min \{w_i, v(S')\}   
    + \sum_{j\in S' \setminus \{i\}} 
     \sum_{\pi \in \PrmL{S'}{j}} 
   \frac{ v^{[S']}(\Prec (\pi,i)\cup \{i\})
    - v^{[S']}(\Prec (\pi,i))}{(|S'|-1)!}
    \right) 
    \\
  &=&\frac{1}{|S'|}
  \left( \min \{w_i, v(S')\}   
    + \sum_{j\in S' \setminus \{i\}} 
     \sum_{\pi \in \PrmL{S'}{j}} 
   \frac{ v(\Prec (\pi,i)\cup \{i\})
    - v(\Prec (\pi,i))}{(|S'|-1)!}
    \right). 
    \\
\end{eqnarray*}

\noindent
We now turn to the final term introduced above
    for each $j \in S'\setminus \{i\}.$

\noindent
(1) In case that  $|S' \setminus \{j\}| \geq 2$ and
    $\sum_{k\in S'\setminus\{j\}}w_k>w_0$, we have that  
\begin{eqnarray*}
\lefteqn{
  \sum_{\pi \in \PrmL{S'}{j}} 
   \frac{ v(\Prec (\pi,i)\cup \{i\})
    - v(\Prec (\pi,i))}{(|S'|-1)!}
}\\
&=&  \sum_{\pi \in \PrmL{S'}{j}}
   \frac{ v^{[S'\setminus \{j\}]}(\Prec (\pi,i)\cup \{i\})
    - v^{[S'\setminus \{j\}]}(\Prec (\pi,i))}{(|S'|-1)!}
=  \sum_{\pi \in \PrmL{S'}{j}}
   \frac{ \delta_{v^{[S'\setminus \{j\}]}} (\pi,i)}{(|S'|-1)!}\\
&=& \frac{1}{|S' \setminus \{j\}|!} 
    \sum_{\pi \in \Pi_{S'\setminus \{j\}}} 
        \delta_{v^{[S'\setminus \{j\}]}} (\pi,i)
= \phi^{[S' \setminus \{j\}]}_i. 
\end{eqnarray*}

\noindent
(2) Consider the case that 
    $|S' \setminus \{j\}|\geq 2$ and $\sum_{k\in S'\setminus\{j\}}w_k\leq w_0.$
As $j \neq i$, every permutation $\pi \in \PrmL{S'}{j}$ satisfies that      
    $\Prec (\pi,i) \subseteq
    \Prec (\pi, i) \cup \{i\} \subseteq S' \setminus \{j\}$
    and thus 
    $0\leq v(\Prec (\pi, i))
    \leq v(\Prec (\pi, i)\cup \{i\} ) 
    \leq v(S' \setminus \{j\})=0$.
From the above, we obtain 
\[
  \sum_{\pi \in \PrmL{S'}{j}} 
   \frac{ v(\Prec (\pi,i)\cup \{i\})
    - v(\Prec (\pi,i))}{(|S'|-1)!}
  =\sum_{\pi \in \PrmL{S'}{j}} 
   \frac{ 0-0}{(|S'|-1)!}
   =0=\phi^{[S' \setminus \{j\}]}_i.
\]

\noindent
(3) Finally, we consider the case 
    where $|S'\setminus \{j\}|=1.$
    It implies that $S'=\{i,j\}$ and 
    $\PrmL{S'}{j}$ contains the unique permutation $(\pi(1),\pi(2))=(i,j)$, 
    from which it follows that
\[
  \sum_{\pi \in \PrmL{S'}{j}} 
   \frac{ v(\Prec (\pi,i)\cup \{i\})
    - v(\Prec (\pi,i))}{(|S'|-1)!}
  = \frac{v(\{i\}) -v(\emptyset )}{1!}
   =v(\{i\})
   =\phi^{[\{i\}]}_i=\phi^{[S' \setminus \{j\}]}_i.
\]    
\end{proof}


==> Proofs-old/ssindex-old.tex <==
\begin{Theorem}\label{Theorem:ssindex}
Consider a bankruptcy game defined by 
    $\BG[E; \Vec{w}]$  
    defined by integer vector $\Vec{w}$  
    and a positive integer estate $E$.
Then the Shapley value of player $i \in N$, denoted by $\phi_i$, satisfies
\[
\phi_i = \sum_{q = w_0+1}^{W} \phi_i^{\langle q \rangle},
\]
where $W = w_1 + \cdots + w_n$.  
Here, $\phi_i^{\langle q \rangle}$ denotes the Shapley–Shubik index of player $i$ 
in the weighted voting game defined by $[q;w_1, w_2, \ldots, w_n]$.
\end{Theorem}



\begin{proof}
From Lemma~\ref{lemma:merg},
\begin{align*}
\phi_i
= \sum_{\pi \in \Pi_N} \Merg(\pi,i) = \sum_{\pi \in \Pi_N} \sum_{q=w_0+1}^W \Mergq(\pi,i) &= \sum_{q=w_0+1}^W \sum_{\pi \in \Pi_N} \Mergq(\pi,i) \\
&= \sum_{q=w_0+1}^W \phi_i^{<q>}.
\end{align*}
\end{proof}


ーーーーーーーーーーーーーーーーーーーーーー
{\color{yellow} 
ーーーーーーーーー old version ーーーーーーーーーーーーーー

\begin{Theorem}\label{Theorem:ssindex2}
Let $\Vec{w}$ be a vector of positive integers, 
    and $E$ be a positive integer satisfying
    $E + 1 < W := \sum_i w_i$. 
Define $\phi^+$ and $\phi$ as the Shapley values corresponding to the bankruptcy games 
$\BG[E+1; \Vec{w}]$ and $\BG[E; \Vec{w}]$, respectively.
The difference between the Shapley values defined above 
    satisfies the identity
\begin{equation} \label{ParametricAnalysis}
    \phi^+ - \phi =\varphi^{\langle W-E \rangle},
\end{equation}
where $\varphi^{\langle W-E \rangle}$ is 
    the Shapley-Shubik index 
    defined by $WVG[W-E;\Vec{w}].$
\end{Theorem}

\begin{proof}
Let $(N,v^+)$, $(N,v)$ and $(N,v^{\langle W-E \rangle})$ 
be characteristic function form games 
    defined by 
    $\BG [E+1;\Vec{w}]$, $\BG [E; \Vec{w}]$ and 
     $\WVG [W-E;\Vec{w}]$, 
    respectively. 
 First, we show the equalities 
    $v^+(S)- v(S)=v^{\langle W-E \rangle} (S)$ 
    $(\forall S \subseteq N).$



If coalition $S$ satisfies 
    $\sum_{i\in S} w_i \leq W-E-1$, 
    then $v^+ (S)=0$, $v(S)=0$ and
    $v^{\langle W-E \rangle} (S)=0$, 
    which implies 
    $v^+(S)- v(S)=0=v^{\langle W-E \rangle} (S).$ 
Consider the case that $\sum_{i\in S} w_i \geq W-E$.
Then, we have that
\[
    v^+(S)-v(S)=
    \left( 
        \left (\sum_{i\in S} w_i \right) - (W-E-1)
    \right)
    -\left( 
        \left( \sum_{i\in S} w_i \right) - (W-E)
    \right) =1=v^{\langle W-E \rangle }(S).
\]

Thus, we have that
    $ v^+=v+v^{\langle W-E \rangle}$
    and the additivity (law of aggregation~\cite{shapley1953value})
of the Shapley value implies the desired result.
\end{proof}

\begin{Cor}
%    Consider a bankruptcy game $(N,v)$ defined by 
%   $\BG[E; \Vec{w}],$  
%    where $\Vec{w}$ is a vector of positive integers 
%    and $E$ is a positive integer satisfying $0<E<W$. 
The Shapley value $\phi$ of $\BG[E; \Vec{w}]$  
    satisfies
$
 \phi= \sum_{q = W-E+1}^{W} \varphi^{\langle q \rangle}.
$
\end{Cor}
% \input{Proofs/ssindex}

\begin{proof}
Let $\phi^{\bullet}$ be the Shapley value of 
     $\BG [1; \Vec{w}].$
Then, by telescoping the sum 
    in equality~(\ref{ParametricAnalysis}), 
    we obtain that 
\begin{eqnarray*}
 \phi &=& \sum_{q=W-E+1}^{W-1} \varphi^{\langle q \rangle}
    +\phi^{\bullet}
    =\sum_{q=W-E+1}^{W-1} \varphi^{\langle q \rangle}
    +\left( \frac{1}{n} \right) (1,1,\ldots ,1) \\
    &=& \sum_{q=W-E+1}^{W-1} \varphi^{\langle q \rangle}
    +\varphi^{\langle W \rangle}
    =\sum_{q=W-E+1}^{W} \varphi^{\langle q \rangle}.
\end{eqnarray*}
\end{proof}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
From the above Corollary, 
    one can compute the Shapley value of a bankruptcy game 
    by executing an algorithm for computing 
    the Shapley–Shubik index of a weighted voting game 
    $E (=W-w_0)$ times.
Furthermore, %as in Aziz~\cite{aziz2013computation}, 
    by modifying the algorithm for computing 
    the Shapley–Shubik index, 
    it may be possible to construct a more efficient method than simply running it $E$ times.

In the following, we describe an algorithm
    based on the dynamic programming technique,
    whose time complexity is bounded by $O(n^2 W)$ for each player. 
The definition of weighted voting game $(N,v_q)$ implies that
\[
    \begin{array}{rcl}
    \phi_i^{\langle q \rangle}&=&\displaystyle 
    \sum_{S\subseteq N \setminus \{i\}}
    \frac{|S|! (n-|S|-1)!}{n!}(v_q(S \cup \{i\})-v_q(S)) \\
    &=& \displaystyle 
    \sum_{t=1}^{n-1} \sum_{w=q-w_i}^{q-1}
    \frac{t! (n-t-1)!}{n!} c_i (w,t),
    \end{array} 
\]
where 
\[
    c_i (w,t)
    =\left\{ \begin{array}{ll} 
    \displaystyle 
    \# \left\{S \subseteq N\setminus \{i\} 
        \left|  \sum_{i \in S} w_i =w \mbox{ and } |S|=t 
        \right. \right\} 
        & (\mbox{ if } 1\leq w\leq W \mbox{ and } 1\leq t \leq n), \\
    0 & (\mbox{otherwise}).
    \end{array} \right.
\]

Theorem~\ref{Theorem:ssindex} implies that
\[
\begin{array}{rcl}
\phi_i %= \sum_{q = w_0+1}^{W} \phi_i^{\langle q \rangle}
&=& \displaystyle 
 \sum_{q = w_0+1}^{W} \sum_{t=1}^{n-1}  \sum_{w=q-w_i}^{q-1}
    \frac{t! (n-t-1)!}{n!} c_i (w,t) \\
&=& \displaystyle 
 \sum_{t=1}^{n-1} 
 \left( 
  \frac{t! (n-t-1)!}{n!}  
    \sum_{w = w_0+1-w_i}^{W-1} 
    \left(
        (\min\{ W, w+w_i\}- \max \{w+1, w_0+1\}) 
        c_i (w,t)
    \right)
 \right),  
 \end{array}
\]  
which allows us to compute the Shapley value $\phi_i$ 
in $O(nW)$ time using
the $W \times n$ matrix $C_i=(c_i(w,t)).$
An ordinary dynamic programming technique gives 
    an algorithm for calculating the matrix $C_i=(c_i(w,t))$
    in $O(n^2 W)$ time (see~\cite{matsui2000survey} for example).
Thus, there exists an algorithm for calculating 
    the Shapley value of a bankruptcy game 
    whose time complexity is bounded by $O(n^2 W)$ for each player. 

}

==> Proofs-old/superadditive.tex <==
\begin{proof}
We prove that $[\forall S, \forall T \subseteq N, 
 S \cap T = \emptyset \rightarrow  v(S)+v(T) \leq v(S \cup T)]$ holds.

\begin{enumerate}
\item  When $-w_0 + \sum\limits_{i \in S \cup T}w_i \leq 0$,
it is clear that $v(S)=v(T)=v(S\cup T) = 0$ holds. Therefore, $v(S)+v(T) \leq v(S \cup T)$
is satisfied.

\item Consider the case where $-w_0 + \sum\limits_{i \in S \cup T}w_i > 0$ is satisfied. 
The assumption $S \cap T=\emptyset$ directly implies the equality $\sum\limits_{i \in S \cup T}w_i = \sum\limits_{i \in S}w_i + \sum\limits_{i \in T}w_i$. 
Therefore, we have that 
\begin{align*}
v(S \cup T) &= -w_0 + \sum\limits_{i \in S \cup T}w_i 
=-w_0 + (\sum\limits_{i \in S}w_i + \sum\limits_{i \in T}w_i) \\
& \geq (-w_0+\sum\limits_{i \in S}w_i) + (-w_0+\sum\limits_{i \in T}w_i) 
=v(S)+v(T).
\end{align*}
\end{enumerate}
\end{proof}

==> Proofs-old/supermodular.tex <==
\begin{proof}
We prove that $[\forall S, \forall T \subseteq N, v(S)+v(T) \leq v(S \cup T) + v(S \cap T)]$ holds.

\begin{enumerate}
\item  When $v(S)=v(T) = 0$,
 the non-negativity of $v(S\cup T)$ and $v(S \cap T)$  leads to the desired inequality.

\item 
When $v(S)>0= v(T)$, 
we have that 
\[
v(S)+v(T)=-w_0 + \sum_{i \in S}w_i +0 
 \leq -w_0 + \sum_{i \in S \cup T}w_i 
 =v(S \cup T)=v(S \cup T) +v(S \cap T).
\]

\item We can similarly address the case that $v(T)>  0=v(S)$ with (2).

\item 
If $v(S)>0$ and $v(T)>0$ hold, 
    it directly implies $v(S \cup T) > 0$ and thus we have that  
\[
\begin{array}{ll}
 v(S \cup T)+ v(S \cap T)  - v(S) - v(T) \\
= \left( -w_0 + \sum\limits_{i \in S \cup T}w_i \right) + v(S \cap T)  
  - \left( -w_0 + \sum\limits_{i \in S}w_i \right) 
  - \left( -w_0 + \sum\limits_{i \in T}w_i \right) \\
 = v(S \cap T) -\left( - w_0 + \sum\limits_{i \in S \cap T}w_i \right) 
 \geq 0.
\end{array}
\]

\end{enumerate}
From the above, $v$ satisfies supermodularity.
\end{proof}

==> Proofs-old/w_0Monotone-old.tex <==

\begin{proof}
In the following proof,  we assume that $(N,v)$ and $(N,v')$ be a pair of rectified linear function games defined by 
$\ReL [w_0; \Vec{w}]$ and  $\ReL [w'_0; \Vec{w}]$
satisfying $w_0+E=w'_0+E'=W$ and thus $w_0 \geq w'_0$.
%Now we show that $\Merg (\pi, i) \leq \MergP (\pi, i)$ for any $(\pi, i) \in \Pi_N \times N$.
Obviously, we have that $\Merg (\pi, i), \MergP (\pi, i) \in [0,w_i]$.
If $w'_0 \leq w(\Prec (\pi, i))$, 
    then the inequality
\[ 
\begin{array}{r@{}l}
\MergP (\pi, i) &= v' (\Prec (\pi, i) \cup \{i\})- v' (\Prec (\pi, i)) \\
    &=(-w'_0 + w(\Prec (\pi, i) \cup \{i\})) -( -w'_0 + w(\Prec (\pi, i) )) 
    = w_i \geq \Merg (\pi, i)
\end{array}
\]
holds.
If $w(\Prec (\pi, i) \cup \{i\}) \leq  w_0$, 
    then we have the following inequality
\[ 
\Merg (\pi, i) = v (\Prec (\pi, i) \cup \{i\})- v(\Prec (\pi, i))
    =0 -0 =0 \leq \MergP (\pi, i).
\]
Lastly, we consider the remained case that
    $w(\Prec (\pi, i)) < w'_0 \leq w_0 < w(\Prec (\pi, i) \cup \{i\})$.
It is easy to see that
\[
\begin{array}{r@{}l}
\MergP (\pi, i) &= v' (\Prec (\pi, i) \cup \{i\})- v'(\Prec (\pi, i))
    = (-w'_0 + w(\Prec (\pi, i) \cup \{i\})) -0 \\
  &\geq   (-w_0 + w(\Prec (\pi, i) \cup \{i\})) -0 
  =  v (\Prec (\pi, i) \cup \{i\})- v(\Prec (\pi, i))
  = \Merg (\pi, i).
\end{array}
\]
\end{proof}
